Just a Second -- Scheduling Thousands of Time-Triggered Streams in Large-Scale Networks

Deterministic real-time communication with bounded delay is an essential requirement for many safety-critical cyber-physical systems, and has received much attention from major standardization bodies such as IEEE and IETF. In particular, Ethernet technology has been extended by time-triggered scheduling mechanisms in standards like TTEthernet and Time-Sensitive Networking. Although the scheduling mechanisms have become part of standards, the traffic planning algorithms to create time-triggered schedules are still an open and challenging research question due to the problem's high complexity. In particular, so-called plug-and-produce scenarios require the ability to extend schedules on the fly within seconds. The need for scalable scheduling and routing algorithms is further supported by large-scale distributed real-time systems like smart energy grids with tight communication requirements. In this paper, we tackle this challenge by proposing two novel algorithms called Hierarchical Heuristic Scheduling (H2S) and Cost-Efficient Lazy Forwarding Scheduling (CELF) to calculate time-triggered schedules for TTEthernet. H2S and CELF are highly efficient and scalable, calculating schedules for more than 45,000 streams on random networks with 1,000 bridges as well as a realistic energy grid network within sub-seconds to seconds.

==> chapters/configuration-graph.tex <==
% !TeX spellcheck = en_US
% !TeX root = ../generic_main.tex

\iffalse

\section{Configuration Graph}
\label{sec:configuration_graph}
\todo[inline]{
	We store our data *TODO find a better term* in a multi-layered graph. 
	This way we have a fast lookup for all necessary information and a comprehensible data model.
}
We model our scheduling problem in a multi-layered graph in three different layers.
A simplified example is illustrated in \Cref{fig:multilayeredconfigurationgraph}.
For sake of clarity, we omit most of the interlayer edges, except for those related to the orange stream and one of its candidate paths.
The stream layer represents the time-triggered streams $F_i \cup R_i$, the candidate route layer specifies the candidate paths $\mathcal{P}^f$ for the streams, and the network layer models the computer network $\mathcal{G}$.
Hence, the vertices and edges represent different concepts depending on the layer.
In the following we will discuss each layer in detail.

\begin{figure}
	\centering
	\includegraphics[width=0.8\linewidth]{pictures/multi_layered_configuration_graph}
	\caption{Multi-layered configuration graph example. Most interlayer links are omitted for brevity. The gray vertices represent network devices. Thereby, the upper two are bridges and the lower three send stations.}
	\label{fig:multilayeredconfigurationgraph}
\end{figure}



\subsection{Network Layer}
\label{sec:configuration_graph:network_layer}

The network layer models the network graph ($\mathcal{G}$) including the network devices' egress ports.
Remember, the network consists of bridges, end stations, and links between them.
Thereby we have two types of vertices in the multi-layered graph: one for network devices (end stations and bridges) displayed as gray vertices in \Cref{fig:multilayeredconfigurationgraph} and egress ports, drawn in dark blue.
The device vertices are used for the routing within the network layer and device specific attributes could be stored here in heterogeneous environments.
Meanwhile, the egress port vertices hold utilization information like the exact forwarding decisions.
This results in a directed bipartite graph where a network device can have multiple egress ports, since the device vertex has an outgoing edge for every of its egress ports and they in turn have a single edge pointing to the next network device.
Full-duplex connections between two devices are modeled by the two egress ports at either end of the cable.

The egress port's utilization is stored as lists of free and reserved slots. 
When a new stream is to be scheduled via a specific candidate route, our scheduler checks for every required egress port if there are enough free slots to schedule the stream in-time.
Or more formally:
\begin{equation}
	\label{eq:precedence_dependency}
	\forall s_i \in \text{Path}: s_i^{\text{end}} + d \leq s_{i+1}^{\text{start}}
\end{equation}
Thereby, $s_i$ stands for the time slot of the $i^{\text{th}}$ hop, where the qualifier ``start'' and ``end'' denote the slots start and end time, respectively.
$d$ is the accumulated delay from switching, propagation and transmission.
If \Cref{eq:precedence_dependency} can be guaranteed, the required free slots are reserved by the new stream.
Thereby, the slots only need to be stored for a hyper cycle since the behavior is repetitive afterwards.
This translates directly to the forwarding table operated by the bridge.


\subsection{Stream Layer}
\label{sec:configuration_graph:stream_layer}

Vertices in the stream layer represent the streams which have to be routed and scheduled.
Every stream is associated with a stream descriptor including the following information: the end systems where the stream origins and its destination, the frame size, the period, and the deadline.
These descriptors can be modeled as vertex labels.
The vertices are not connected to other vertices of the stream layer but have only edges to vertices in the routing layer.
These edges connect the stream layer vertex to its candidate routes in the routing layer.


\subsection{Candidate Routes Layer}
\label{sec:configuration_graph:routing_layer}


The routing layer hosts a larger amount of vertices, each representing a candidate route for a specific stream.
Such a routing vertex has an undirected edge to its corresponding stream vertex as discussed before, and it has edges to the egress port vertices which are part of its path in the network layer.
Thus, the routing layer connects to both, the stream and the network layer.
Due to this connection potential conflicts between candidate paths can be found easily.

\fi % Config Graph Chapter is soft removed


